BirdSLAM: Monocular Multibody SLAM in Bird's-Eye View

In this paper, we present BirdSLAM, a novel simultaneous localization and mapping (SLAM) system for the challenging scenario of autonomous driving platforms equipped with only a monocular camera. BirdSLAM tackles challenges faced by other monocular SLAM systems (such as scale ambiguity in monocular reconstruction, dynamic object localization, and uncertainty in feature representation) by using an orthographic (bird's-eye) view as the configuration space in which localization and mapping are performed. By assuming only the height of the ego-camera above the ground, BirdSLAM leverages single-view metrology cues to accurately localize the ego-vehicle and all other traffic participants in bird's-eye view. We demonstrate that our system outperforms prior work that uses strictly greater information, and highlight the relevance of each design decision via an ablation analysis.

==> 03pipeline.tex <==
\section{PIPELINE}
\label{sec:pipeline}

\MK{We are not saying how one module input feeds to another. We are explaining them as standalone modules without mentioning the linkages}

\birdslam{} takes in a stream of monocular RGB images as input. We further divide our pipeline into the following modules:

% -------------------------------------------%
\subsection{Dynamic \bev{} Initialisation}
\label{subsec:pipeline_dynamic}
This module gets tight bounding box in \bev{} for dynamic participants in the frame (~\cf Fig. \tbd{}) as explained in Sec. \ref{subsec:vehloc}. The center of this tight bounding boxes are registered with ego motion and is used as input for GPML trajectory prediction (~\cf Sec. \ref{subsec:pipeline_gpml}).
% -------------------------------------------%

%--------------------------------------------%
\subsection{Static \bev{} Initialisation}
\label{subsec:pipeline_static}
In this module, we track static feature points between the scenes by using ORB\cite{orbslam2} correspondences on road as described in Sec. \ref{subsec:statpoint}. The output of this module is directly used as input in pose-graph optimizer (~\cf Sec. \ref{subsec:pipeline_pose_graph}).
%--------------------------------------------%

% ----------------------------------------%
\subsection{Odometry Initialisation}
\label{subsec:pipeline_ego}
\todo{Gokul}{Write short summary of Odometry Module}
% ----------------------------------------%

% optional
%----------------------------------------%
% \subsection{Road Layout Generator}
% \label{subsec:pipeline_road_layout}
% Road Layout is generated by using approximate \bev{} occupancy maps of lane boundaries and road(~\cf Sec. \tbd{}) as input to ENet\cite{enet} to produce amodal complete road layout and lane boundaries layout separately which is then segmented into separate lanes using morphological techniques (opening and closing) and hough line fitting.
% ---------------------------------------%

% -------------------------------------- %
\subsection{Next Instance Predictor}
\label{subsec:pipeline_gpml}
\todo{Gokul}{Write short summary of GP Prediction Module}
% -------------------------------------- %


%----------------------------------------%
\subsection{Orthographic Pose Graph Optimizer}
\label{subsec:pipeline_pose_graph}
\todo{Gokul}{Write short summary of Pose Graph Module}
% ---------------------------------------%


Finally, we get multibody localizations and trajectories along with road and lane estimates in a single unified global frame in \bev{}.

